OOOE: Only-One-Object-Exists Assumption to Find Very Small Objects in Chest Radiographs

The accurate localization of inserted medical tubes and parts of human anatomy is a common problem when analyzing chest radiographs and something deep neural networks could potentially automate. However, many foreign objects like tubes and various anatomical structures are small in comparison to the entire chest X-ray, which leads to severely unbalanced data and makes training deep neural networks difficult. In this paper, we present a simple yet effective `Only-One-Object-Exists' (OOOE) assumption to improve the deep network's ability to localize small landmarks in chest radiographs. The OOOE enables us to recast the localization problem as a classification problem and we can replace commonly used continuous regression techniques with a multi-class discrete objective. We validate our approach using a large scale proprietary dataset of over 100K radiographs as well as publicly available RANZCR-CLiP Kaggle Challenge dataset and show that our method consistently outperforms commonly used regression-based detection models as well as commonly used pixel-wise classification methods. Additionally, we find that the method using the OOOE assumption generalizes to multiple detection problems in chest X-rays and the resulting model shows state-of-the-art performance on detecting various tube tips inserted to the patient as well as patient anatomy.

==> body/02_related_work_.tex <==
\section{Related Work}

\subsection{Landmark Detection}


\subsection{ETTube Malpositioning Detection}
\ett~malpositioning detection is one of the most easily applicable task for the point detection~\cite{frid2019simul,kara2021ett}.
Frid-Adar~\etal~\cite{frid2019simul} propose to generate synthetic data to augment \ett~to increase the detection performance for \ett. 
This method proves their synthesizing method successfully enhances the \ett~classification performance. 
However, they does not neither propose the malpositioning detection method nor proves the detection and segmentation performance gain.

% Small object detection 
Related to our problem is the problem of small object detection \cite{chen2016r, tong2020recent}. Tong et al. \cite{tong2020recent} survey recent work on using object detection architectures for small objects and identify five general approaches: multi-scale feature learning, data augmentation, training strategy, context-based detection and GAN-based detection \cite{tong2020recent}. However, methods typically do not make any assumptions on the number of objects or try to reduce the problem to that of point detection.

% Landmark/point detection
Another similar problem is that of landmark localization \cite{honari2018improving}. However, no assumptions are typically made about the number of objects that are present. 

Kara \etal~\cite{kara2021ett} adopts a cascade method to localize carina and \ett.
They delicately design the pipeline with three different stages. 
Firstly, carina location is regressed as a point. 
Then, \ett~presence or absence is determined with an input of a patch cropped based on the carina location.
Lastly, the \ett~tip point is regressed along with the carina location refinement.
This approach proposes the entire pipeline foor the \ett~malpositioning detection by point detection methodology.

The biggest difference between our approach and the previous work is that we transform the regression problem into classification problem. 
The discriminative learning is well-known to outperform regression learning methods for deep learning method~\cite{oh2017color,li2017kp_cls,li2018bin_cls,su20153d_cls}. 
In this paper, we proves that the discriminative method is also effective for the point detection problem. 


==> body/03_method_.tex <==
\section{Methods}

\input{resources/figures/head_outputs}
As mentioned in the introduction, we address the problem of detecting small objects in an image, using the assumption that they occur once and only once. We also observe that small objects, such as the tip of a tube or a certain landmark of the anatomy, can essentially be represented as a single point in an image. 

% Then, the small object detection problem can be cast as a point detection problem such that:
% problem definition
% Given an image $\img$, our task is to find a small object in the image, which is represented as a single point.
% % Note that one of property in the point detection is that the point can be represented one pixel in a image (\ie~\textbf{only-one-object-exists assumption)}. 
% Our deep neural network solution for the task consists of two parts: a feature extractor $\featureExtractor$ and a detection head $\head$. The point detection is formulated as following:

%\begin{equation}
%     \hat{\pred} = \head(\featureExtractor(\img)),
%\end{equation}
%where $\featureExtractor$ extracts features from the input $\img$, $\head$ is the detection head that produces point prediction $\hat{\pred}$. $\featureExtractor$ and $\head$ can be implemented using common deep neural network architectures.

%Let $X = \featureExtractor(\img), X \in \mathbb{R}^{C \times H \times W}$ be the output of the feature extractor. 

% Our objective is to find optimal parameters $\theta^*$ for the feature extractor and detection head to minimize a loss function $\mathcal{L}$ for the model output and ground-truth:
% \begin{equation}
%     \theta^* = \argmin_{\theta} \mathcal{L}(\pred,\hat{\pred}),
% \end{equation}
% where $\pred$ is the ground truth and $\hat{\pred}$ is the model prediction.

% In the following subsections, we describe our \textit{spatial softmax} and other commonly used methods including \textit{regression} and \textit{pixel-wise classification} based solutions to this problem. \Fref{fig:head_outputs} summarizes the differences between the three types of approaches.
% While our approach can be regarded as a point classification method along with the pixel-wise classification in that it casts the localization problem to classification problem, ours incorporates the OOOE assumption into the point classification.

In the following subsections, we introduce our OOOE inspired \textit{spatial softmax} approach and compare it to other common \textit{regression} and \textit{pixel-wise classification} based solutions to this problem. \Fref{fig:head_outputs} summarizes the differences between the three types of approaches.

% The point detection problem is commonly solved as either a  \textit{regression} or a \textit{classification} problem.
% In the classification method, we can adopt two different output activation strategies: a \textit{pixel-wise classification} and a \textit{spatial softmax}.
% \Fref{fig:head_outputs} compares the three different solutions for the problem. In this section, we describe how we implement each learning strategies in details.

\subsection{Point Regression}
\label{sec:regression}
Regression based approaches such as \cite{kara2021ett} produce a 2 channel output given $\featureExtractor(\img)$ such that $\hat{\pred}=[\hat{\pred}_1, \hat{\pred}_2]$.
%The point regression method is a general point detection method~\cite{kara2021ett}. From feature map derived from the feature extractor, a linear regression head outputs 2 channels for each point $\hat{\pred}=[\hat{\pred}_1, \hat{\pred}_2]$ after max-pooling the feature map.
The model is trained by minimizing the mean-square-error (MSE) between the predicted $\hat{\pred}$ and ground truth $\pred$ point location. 
% \begin{equation}
%     \mathcal{L}(\pred, \hat{\pred}) = \frac{1}{2}\sum_{i=1}^{2}||\pred_i - \hat{\pred}_i||_2.
% \end{equation}

\subsection{Point Classification}
\label{sec:classification}
Classification based methods have outperformed regression approaches in multiple detection problems ~\cite{oh2017color,li2017kp_cls,li2018bin_cls,su20153d_cls,jeon2020pose_att,jakab2018unsup_keypoint}. 
The key intuition behind such methods is that by discretizing the continuous prediction space, the optimization of the network becomes easier and thus detection model reaches higher performance.
%Also, most of key point detection methods adopt discriminative manner for the point detection~\cite{jeon2020pose_att,jakab2018unsup_keypoint}.
%To exploit the discriminative power of deep learning methods, we adopt pixel classification from a feature map.
In a classification setup, the model outputs an activation map $\hat{\pred} \in \mathbb{R}^{H \times W}$ where the value located at $(i, j)$ is $\hat{\pred}_{ij} = \head(\feature_{ij})$ and $\featureExtractor(\img) = \featureMap = [\feature_{11}, \feature_{12}, ... , \feature_\textit{WH}]$.
The pixel classification can be achieved through two different output activation strategies: \textit{pixel-wise classification} and \textit{spatial softmax}.

\textbf{Pixel-wise classification} is widely used for image segmentation tasks~\cite{ronneberger2015unet,long2015fcn} where each pixel in a feature map is independently classified as the most probable class. 
Here, we perform binary classification for each class for all pixel locations similar to \cite{ronneberger2015unet,long2015fcn} and the model is trained end-to-end by minimizing pixel-wise binary cross entropy.

% For the output activation, the sigmoid function $\sigmoid(x) = \frac{1}{1+e^{-x}}$ is used.
% The loss is formulated as following:
% \begin{equation}
%     \mathcal{L}(\pred, \hat{\pred}) = \frac{1}{HW}\sum_{j=1}^{H}\sum_{i=1}^{W} - \mathbbm{1}_{\pred=(i,j)} \log \sigmoid(\hat{\pred}_{ij}) - (1 - \mathbbm{1}_{\pred=(i,j)} )\log (1 - \sigmoid(\hat{\pred}_{ij})),
% \end{equation}
% where $\mathbbm{1}_{\pred=(i,j)}$ denotes 1 if $\pred = (i, j)$.

\textbf{Spatial softmax} is an output activation function commonly used for landmark detection tasks~\cite{jakab2018unsup_keypoint,jeon2020pose_att}.
They used the spatial softmax to represent a landmark from network outputs and proved it outperforms simple regression method to localize accurate landmarks. 
In this paper, we propose to use this loss for the detection of single, small objects in chest radiographs. 

The spatial softmax allows the detection head to produce a relative probability for each pixel, compared to all other pixels in the image. This satisfies the OOOE assumption we make in this paper, that states one and only one instance of the object is present in the image. 

The most probable pixel in a feature map is activated by applying the softmax function along the spatial axis of the image. Mathematically, the spatial softmax $\spatialSoftmax$ is defined as follows:
\begin{equation}
    \spatialSoftmax(\pred)_{ij} = \frac{e^{\pred_{ij}}}{\sum_{n=1}^H\sum_{m=1}^{W} e^{\pred_{nm}}}.
\end{equation}
The model is finally optimized by the negative log-likelihood loss as following:
\begin{equation}
    \mathcal{L}(\pred, \hat{\pred}) = \frac{1}{HW}\sum_{j=1}^{H}\sum_{i=1}^{W} - \mathbbm{1}_{\pred=(i,j)} \log (\spatialSoftmax(\hat{\pred})_{ij}),
\end{equation}
where $\mathbbm{1}_{\pred=(i,j)}$ outputs 1 if $\pred = (i, j)$.

==> resources/tables/carina.tex <==
\begin{table*}[t]
\centering
\setlength{\tabcolsep}{7pt}
\caption{Carina Detection Scores}
\label{table:carina}
\begin{tabular}{l|ccc}
\toprule
Split  &  Regression &  Pixel-wise Classification &  Spatial Softmax \\
\midrule
Point-internal       &        90.7 &                96.3 &             97.0 \\
Point-small          &        79.8 &                97.5 &             98.0 \\
Point-large          &        91.3 &                95.1 &             95.9 \\
Point-internal-ttube &        91.5 &                96.4 &             96.9 \\
Point-large-ttube    &        90.4 &                95.0 &             96.0 \\
\bottomrule
\end{tabular}
\end{table*}

==> resources/tables/ettube-tip.tex <==
\begin{table*}[t]
\centering
\setlength{\tabcolsep}{7pt}
\caption{ET-Tube Tip Detection Scores}
\label{table:ettube-tip}
\begin{tabular}{l|ccc}
\toprule
Split  &  Regression &  Pixel-wise Classification &  Spatial Softmax \\
\midrule
Point-internal       &        80.5 &                93.4 &             95.7 \\
Point-small          &        60.9 &                81.0 &             82.7 \\
Point-large          &        74.3 &                78.6 &             70.0 \\
Point-internal-ttube &        85.7 &                93.3 &             96.1 \\
Point-large-ttube    &        80.8 &                83.2 &             83.9 \\
\bottomrule
\end{tabular}
\end{table*}

==> resources/tables/performance.tex <==
\begin{table}
\centering
\caption{ }
\small
\label{table:performance-}
\begin{tabular}{l|c|c|c|c|c|c|c|c|c|c|c|c}
\toprule
{} & \multicolumn{6}{c|}{Carina} &  \multicolumn{6}{c}{ETT Tip} \\
\midrule
&    \multicolumn{2}{c|}{Reg}  & \multicolumn{2}{c|}{PC} & \multicolumn{2}{c|}{SS} &  \multicolumn{2}{c|}{Reg} & \multicolumn{2}{c|}{PC} &  \multicolumn{2}{c}{SS}      \\

\midrule
&    AUC &       95\% CI &        AUC &     95\% CI &        AUC &     95\% CI &     AUC &     95\% CI &        AUC &      95\% CI &         AUC &      95\% CI  \\  
\midrule

\internalExp   &   74.5 &  73.7-75.3 &       85.7 &  85.0-86.4 &       86.8 &  86.1-87.5 &    69.1 &  67.1-70.9 &       82.9 &   81.1-84.3 &        87.4 &   86.3-88.8 \\
\smallEconnExp &   46.5 &    45.2-47.7 &       71.4 &  70.6-72.3 &       72.1 &  71.1-72.9 &    35.1 &  32.8-37.9 &       60.8 &   58.7-63.6 &        73.6 &   71.7-75.3 \\
\smallExp      &   59.2 &    57.8-60.6 &       87.0 &  86.4-87.5 &       89.3 &  88.7-89.9 &    42.4 &  41.0-44.0 &       67.5 &   65.8-69.1 &        70.4 &   68.8-71.8 \\
\largeExp      &   69.1 &    68.2-70.2 &       79.2 &  78.4-79.8 &       81.1 &  80.7-81.6 &    67.2 &  65.5-68.8 &       75.1 &   73.1-76.9 &        76.8 &   74.9-78.7 \\
\bottomrule
\end{tabular}
\end{table}
